Probing the Cosmic Baryon Distribution and the Impact of Active Galactic Nuclei Feedback with Fast Radio Bursts in CROCODILE Simulation

We investigate the Missing Baryon problem using Fast Radio Bursts (FRBs) to trace cosmic baryons. Our CROCODILE simulations, performed with the GADGET3/4-OSAKA smoothed particle hydrodynamics code, include star formation, supernova (SN) and active galactic nuclei (AGN) feedback. We generate light cones from large-scale structure simulations to compute gas density profiles and dispersion measures (DMs) measurable by FRBs. Our results show that AGN feedback reduces central gas densities in halos, reshaping the boundary between the circumgalactic medium (CGM) and intergalactic medium (IGM). Zoom-in simulations reveal that AGN feedback significantly modulates the DM contributions from foreground halos along different sightlines. Using the DM-redshift (DM-z) relation up to z=1, we constrain the diffuse baryon mass fraction at z = 1 to f_diff = 0.865 (+0.101, -0.165) (fiducial) and f_diff = 0.856 (+0.101, -0.162) (NoBH), which include contributions from both IGM (f_IGM) and halos (f_Halos), serving as upper limits. We further separate and quantify the redshift evolution of f_CGM, f_IGM, and f_diff using both phase-based and structure-based definitions. From an observational perspective, we also distinguish the line-of-sight averaged quantity < f_{diff,obs} > from the intrinsic redshift-evolving f_diff(z), reflecting the statistical nature of FRB-based measurements. Our study provides a framework for understanding baryon distribution across cosmic structures, FRB host galaxies, and the role of AGN in shaping foreground DM contributions.

==> Bibtex.tex <==
\begin{thebibliography}{}
\expandafter\ifx\csname natexlab\endcsname\relax\def\natexlab#1{#1}\fi
\providecommand{\url}[1]{\href{#1}{#1}}
\providecommand{\dodoi}[1]{doi:~\href{http://doi.org/#1}{\nolinkurl{#1}}}
\providecommand{\doeprint}[1]{\href{http://ascl.net/#1}{\nolinkurl{http://ascl.net/#1}}}
\providecommand{\doarXiv}[1]{\href{https://arxiv.org/abs/#1}{\nolinkurl{https://arxiv.org/abs/#1}}}
% 参考文献部分
\bibitem[Cen(2012)]{Cen2012ApJ...753...17C} Cen, R.\ 2012, \apj, 753, 17. doi:10.1088/0004-637X/753/1/17

\bibitem[Cen \& Ostriker(1999)]{CO1999ApJ...514....1C} Cen, R. \& Ostriker, J.~P.\ 1999, \apj, 514, 1. doi:10.1086/306949

\bibitem[CHIME/FRB Collaboration et al.(2021)]{2021ApJS..257...59C} CHIME/FRB Collaboration, Amiri, M., Andersen, B.~C., et al.\ 2021, \apjs, 257, 59. doi:10.3847/1538-4365/ac33ab

\bibitem[Chime/FRB Collaboration et al.(2023)]{2023ApJS..264...53C} Chime/Frb Collaboration, Amiri, M., Andersen, B.~C., et al.\ 2023, \apjs, 264, 53. doi:10.3847/1538-4365/acb54c


\bibitem[Danforth \& Shull(2005)]{DS2005ApJ...624..555D} Danforth, C.~W. \& Shull, J.~M.\ 2005, \apj, 624, 555. doi:10.1086/429285

\bibitem[Danforth \& Shull(2008)]{DS2008ApJ...679..194D} Danforth, C.~W. \& Shull, J.~M.\ 2008, \apj, 679, 194. doi:10.1086/587127

\bibitem[Dav{\'e} et al.(2001)]{Dave2001ApJ...552..473D} Dav{\'e}, R., Cen, R., Ostriker, J.~P., et al.\ 2001, \apj, 552, 473. doi:10.1086/320548

\bibitem[Fukushima et al.(2023)]{Fukushima2023MNRAS.525.3760F} Fukushima, K., Nagamine, K., \& Shimizu, I.\ 2023, \mnras, 525, 3760. doi:10.1093/mnras/stad2526

\bibitem[Khrykin et al.(2024)]{Khrykin2024arXiv240200505K} Khrykin, I.~S., Ata, M., Lee, K.-G., et al.\ 2024, arXiv:2402.00505. doi:10.48550/arXiv.2402.00505

\bibitem[Khrykin et al.(2024)]{Khrykin2024MNRAS.529..537K} Khrykin, I.~S., Sorini, D., Lee, K.-G., et al.\ 2024, \mnras, 529, 537. doi:10.1093/mnras/stae525

\bibitem[Lee et al.(2022)]{Lee2022} Lee, K.-G., Ata, M., Khrykin, I.~S., et al.\ 2022, \apj, 928, 9. doi:10.3847/1538-4357/ac4f62

\bibitem[Lee et al.(2023)]{Lee2023} Lee, K.-G., Khrykin, I.~S., Simha, S., et al.\ 2023, \apjl, 954, L7. doi:10.3847/2041-8213/acefb5

\bibitem[Lorimer et al.(2007)]{Lorimer2007} Lorimer, D.~R., Bailes, M., McLaughlin, M.~A., et al.\ 2007, Science, 318, 777. doi:10.1126/science.1147532

\bibitem[Macquart et al.(2020)]{Macquart2020Nature} Macquart, J.-P., Prochaska, J.~X., McQuinn, M., et al.\ 2020, \nat, 581, 391. doi:10.1038/s41586-020-2300-2

\bibitem[Nicastro et al.(2005a)]{Nicastro2005a} Nicastro, F., Mathur, S., Elvis, M., et al.\ 2005a, \nat, 433, 495. doi:10.1038/nature03245

\bibitem[Nicastro et al.(2005b)]{Nicastro2005b} Nicastro, F., Mathur, S., Elvis, M., et al.\ 2005b, \apj, 629, 700. doi:10.1086/431270

\bibitem[Oku et al.(2022)]{Oku2022} Oku, Y., Tomida, K., Nagamine, K., et al.\ 2022, \apjs, 262, 9. doi:10.3847/1538-4365/ac77ff

\bibitem[Prochaska et al.(2011)]{Prochaska2011ApJ...740...91P} Prochaska, J.~X., Weiner, B., Chen, H.-W., et al.\ 2011, \apj, 740, 91. doi:10.1088/0004-637X/740/2/91

\bibitem[Salucci \& Persic(1999)]{Salucci1999MNRAS.309..923S} Salucci, P. \& Persic, M.\ 1999, \mnras, 309, 923. doi:10.1046/j.1365-8711.1999.02913.x

\bibitem[Reiprich \& B{\"o}hringer(2002)]{Reiprich2002ApJ...567..716R} Reiprich, T.~H. \& B{\"o}hringer, H.\ 2002, \apj, 567, 716. doi:10.1086/338753

\bibitem[Rybicki \& Lightman(1979)]{RL1979rpa..book.....R} Rybicki, G.~B. \& Lightman, A.~P.\ 1979, A Wiley-Interscience Publication, New York: Wiley, 1979

\bibitem[Richter et al.(2006)]{Richter2006} Richter, P., Savage, B.~D., Sembach, K.~R., et al.\ 2006, \aap, 445, 827. doi:10.1051/0004-6361:20053636

\bibitem[Richter et al.(2004)]{Richter2004} Richter, P., Savage, B.~D., Tripp, T.~M., et al.\ 2004, \apjs, 153, 165. doi:10.1086/421297

\bibitem[Simha et al.(2023)]{Simha2023ApJ...954...71S} Simha, S., Lee, K.-G., Prochaska, J.~X., et al.\ 2023, \apj, 954, 71. doi:10.3847/1538-4357/ace324

\bibitem[Shimizu et al.(2019)]{Shimizu2019MNRAS.484.2632S} Shimizu, I., Todoroki, K., Yajima, H., et al.\ 2019, \mnras, 484, 2632. doi:10.1093/mnras/stz098

\bibitem[Sorini et al.(2022)]{Sorini2022MNRAS.516..883S} Sorini, D., Dav{\'e}, R., Cui, W., et al.\ 2022, \mnras, 516, 883. doi:10.1093/mnras/stac2214

\bibitem[So{\l}tan(2006)]{Sotan2006A&A...460...59S} So{\l}tan, A.~M.\ 2006, \aap, 460, 59. doi:10.1051/0004-6361:20065431

\bibitem[Thornton et al.(2013)]{Thornton2013} Thornton, D., Stappers, B., Bailes, M., et al.\ 2013, Science, 341, 53. doi:10.1126/science.1236789

\bibitem[Tilton et al.(2012)]{Tilton2012ApJ...759..112T} Tilton, E.~M., Danforth, C.~W., Shull, J.~M., et al.\ 2012, \apj, 759, 112. doi:10.1088/0004-637X/759/2/112

\bibitem[Tripp et al.(2006)]{Tripp2006ASPC..348..341T} Tripp, T.~M., Bowen, D.~V., Sembach, K.~R., et al.\ 2006, Astrophysics in the Far Ultraviolet: Five Years of Discovery with FUSE, 348, 341

\bibitem[Wang \& Wei(2023)]{Wang2023ApJ...944...50W} Wang, B. \& Wei, J.-J.\ 2023, \apj, 944, 50. doi:10.3847/1538-4357/acb2c8

\bibitem[Yang et al.(2022)]{Yang2022ApJ...940L..29Y} Yang, K.~B., Wu, Q., \& Wang, F.~Y.\ 2022, \apjl, 940, L29. doi:10.3847/2041-8213/aca145

\bibitem[Yao et al.(2012)]{Yao2012ApJ...746..166Y} Yao, Y., Shull, J.~M., Wang, Q.~D., et al.\ 2012, \apj, 746, 166. doi:10.1088/0004-637X/746/2/166

\bibitem[Yoshikawa et al.(2001)]{Yoshikawa2001ApJ...558..520Y} Yoshikawa, K., Taruya, A., Jing, Y.~P., et al.\ 2001, \apj, 558, 520. doi:10.1086/322445

\bibitem[Zwaan et al.(2003)]{Zwaan2003AJ....125.2842Z} Zwaan, M.~A., Staveley-Smith, L., Koribalski, B.~S., et al.\ 2003, \aj, 125, 2842. doi:10.1086/374944

\end{thebibliography}{}
